A Dynamic Mode Decomposition Extension for the Forecasting of Parametric Dynamical Systems

Dynamic mode decomposition (DMD) has recently become a popular tool for the non-intrusive analysis of dynamical systems. Exploiting Proper Orthogonal Decomposition (POD) as a dimensionality reduction technique, DMD is able to approximate a dynamical system as a sum of spatial basis evolving linearly in time, thus enabling a better understanding of the physical phenomena and forecasting of future time instants. In this work we propose an extension of DMD to parameterized dynamical systems, focusing on the future forecasting of the output of interest in a parametric context. Initially all the snapshots -- for different parameters and different time instants -- are projected to a reduced space; then DMD, or one of its variants, is employed to approximate reduced snapshots for future time instants. Exploiting the low dimension of the reduced space the predicted reduced snapshots are then combined using regression techniques, thus enabling the possibility to approximate any untested parametric configuration in future. This paper depicts in detail the algorithmic core of this method; we also present and discuss three test cases for our algorithm: a simple dynamical system with a linear parameter dependency, a heat problem with nonlinear parameter dependency and a fluid dynamics problem with nonlinear parameter dependency.

==> sections/notation.tex <==
\RA{
\small
\subsubsection*{Abbreviations}~\\[5pt]
\smallskip
\begin{tabular}{ll}
ROM & Reduced Order Model \\
PDE & Partial Differential Equation \\
POD & Proper Orthogonal Decomposition \\
DMD & Dynamic Mode Decomposition \\
HODMD & Higher-order Dynamic Mode Decomposition \\
\end{tabular}
\subsubsection*{Symbols}~\\[5pt]
\begin{tabular}{ll}
$\mathbb P$ & parameter space  \\
$p$ & number of parameters \\
$N$ & number of time instants\\
$m$ & number of spatial degrees of freedom\\
$n$ & reduced (or latent) dimension \\
$\mathbf x^{\mu_i}_{t^k}$ & high-fidelity snapshot for $\mu_i$ at time $t^k$ \\
$\widetilde{\mathbf x}^{\mu_i}_{t^k}$ & reduced snapshot for $\mu_i$ at time $t^k$ \\
$\hat{\mathbf x}^{\mu_i}_{t^k}$ & approximated high-dimensional snapshot for $\mu_i$ at time $t^k$ \\
$\tilde{\mathbf A}$ & monolithic DMD operator\\
$\{\tilde{\mathbf A}^{\mu_i}\}_{i=1}^p$ & partitioned DMD operators\\
\end{tabular}
}

==> sections/preamble.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{A DMD extension for the forecasting of parametric dynamical systems}{F. Andreuzzi, N. Demo, and G. Rozza}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A dynamic mode decomposition extension for the forecasting of parametric dynamical systems\thanks{Submitted to the editors DATE.}}
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Francesco Andreuzzi\thanks{Mathematics Area, Mathlab, Via Bonomea 265, I-34136 Trieste, Italy
  (\email{francesco.andreuzzi@sissa.it}).}
\and Nicola Demo\thanks{Mathematics Area, Mathlab, Via Bonomea 265, I-34136 Trieste, Italy
  (\email{nicola.demo@sissa.it}).}
\and Gianluigi Rozza\thanks{Mathematics Area, Mathlab, Via Bonomea 265, I-34136 Trieste, Italy
  (\email{gianluigi.rozza@sissa.it}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\sech}{sech}


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

\usepackage{subcaption}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{mathtools}
\usepackage{multicol}
\usepackage{comment}
\usepackage{booktabs}
\usepackage{amssymb}
\usepackage{url}
\usepackage{bm}
\usepackage[a4paper,left=3cm,right=3cm,top=2.5cm,bottom=2.5cm]{geometry}
\usepackage{amsmath}
\usepackage{multirow}
\usepackage{float}
\usepackage{tabularx}
\usepackage{enumerate}
\usepackage{array}
\usepackage{xspace}
\usepackage{tikz}
\usepackage[export]{adjustbox}
\usepackage{tikzsymbols}

\usetikzlibrary{external}
\tikzexternalize

\numberwithin{equation}{section}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{fillbetween}
\pgfplotsset{compat=1.5}
\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,%
    decorations.pathreplacing,decorations.pathmorphing,shapes,%
    matrix,shapes.symbols, decorations.markings, patterns,fit,quotes,%
    arrows.meta, spy}

\usepackage{xcolor}
\definecolor{Gray}{gray}{0.9}

\usepackage{hyperref}
\usepackage{siunitx}

\usepackage[bottom]{footmisc}


\graphicspath{{figures/}}

\newcommand{\TODO}[1]{{\color{red}#1}}
\newcommand{\mupar}{\ensuremath{\boldsymbol{\mu}}}
\newcommand{\etapar}{\ensuremath{\boldsymbol{\eta}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\fulldim}{\ensuremath{\mathcal{N}}}
\newcommand{\reddim}{\ensuremath{N}}
\newcommand{\pardim}{\ensuremath{m}}

\newcommand{\fullspace}{\ensuremath{\mathbb{X}^\fulldim}}
\newcommand{\redspace}{\ensuremath{\mathbb{X}^\fulldim_\reddim}}
\newcommand{\parspace}{\ensuremath{{\bf P}}}
\newcommand{\Xtrain}{\ensuremath{\mathbf{X}}}
\newcommand{\Xtest}{\ensuremath{\mathbf{\Bar{X}}}}
\newcommand{\ytrain}{\ensuremath{\mathbf{y}}}
\newcommand{\ytest}{\ensuremath{\mathbf{\Bar{y}}}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rvline}{\hspace*{-\arraycolsep}\vline\hspace*{-\arraycolsep}}
\newcommand{\ntrain}{p}
\newcommand{\timedim}{N}
\newcommand{\spacedim}{m}
\newcommand{\npod}{n}
\newcommand{\nclusters}{s}
\newcommand{\paramdim}{q}

\newcommand{\RA}[1]{{\color{blue}#1}}
\newcommand{\RB}[1]{{\color{red}#1}}
\newcommand{\Rall}[1]{{\color{green}#1}}

\newcommand{\matr}[1]{\mathbf{#1}}

